BiomedParse: a biomedical foundation model for image parsing of everything everywhere all at once

Biomedical image analysis is fundamental for biomedical discovery in cell biology, pathology, radiology, and many other biomedical domains. Holistic image analysis comprises interdependent subtasks such as segmentation, detection, and recognition of relevant objects. Here, we propose BiomedParse, a biomedical foundation model for imaging parsing that can jointly conduct segmentation, detection, and recognition for 82 object types across 9 imaging modalities. Through joint learning, we can improve accuracy for individual tasks and enable novel applications such as segmenting all relevant objects in an image through a text prompt, rather than requiring users to laboriously specify the bounding box for each object. We leveraged readily available natural-language labels or descriptions accompanying those datasets and use GPT-4 to harmonize the noisy, unstructured text information with established biomedical object ontologies. We created a large dataset comprising over six million triples of image, segmentation mask, and textual description. On image segmentation, we showed that BiomedParse is broadly applicable, outperforming state-of-the-art methods on 102,855 test image-mask-label triples across 9 imaging modalities (everything). On object detection, which aims to locate a specific object of interest, BiomedParse again attained state-of-the-art performance, especially on objects with irregular shapes (everywhere). On object recognition, which aims to identify all objects in a given image along with their semantic types, we showed that BiomedParse can simultaneously segment and label all biomedical objects in an image (all at once). In summary, BiomedParse is an all-in-one tool for biomedical image analysis by jointly solving segmentation, detection, and recognition for all major biomedical image modalities, paving the path for efficient and accurate image-based biomedical discovery.

==> nbt_sec/cover_letter.tex <==
Email to Anne Dörr, Nat Biotech
anne.doerr@nature.com

Dear Dr. Dörr,

We would like to gauge your interest in our manuscript for publication in Nature Biotechnology. We proposed a new biomedical foundation model for holistic image analysis using GPT-4 and generative AI.

Background: Biomedical image analysis is fundamental for biomedical discovery. A holistic analysis comprises interdependent subtasks such as segmentation, object detection, and recognition. However, existing methods for biomedical image analysis tend to ignore their dependencies and tackle these tasks separately using specialized tools, resulting in labor intensive development and suboptimal performance.

Key contribution: To address this long-standing problem, we developed BiomedParse, a biomedical imaging foundation model that simultaneously addresses image segmentation, object detection, and object recognition. BiomedParse is designed as a GPT-style chatbot that allows biologists to talk to the image for their needs. This is unprecedented because biologists no longer need to run any specialized software or label anything in the image (e.g., drawing a bounding box for segmentation). In fact, biologists can identify and locate all objects in the image without even taking a look at the image. Our model, for the first time, makes biomedical image analysis completely automated and intelligent. 

Key novelty: BiomedParse achieves this through a new analysis paradigm called image parsing powered by a biomedical foundation model. Our image parsing framework learns to jointly perform segmentation, object detection, and recognition by leveraging their interdependencies (e.g., the semantic class for a segmented object). This not only makes it more accurate but also enables it to analyze a new image with minimal or even zero user efforts, dramatically decreasing the user effort for all tasks in image analysis. 

Key technical advances: Image parsing used to be developed based on the Bayesian framework for image analysis 20 years ago, but was then quickly replaced by deep learning. We renovated image parsing by integrating GPT-4 into it, resulting in a model that can simultaneously understand images and text, corresponding to the "everything everywhere all at once" in our title.

Concretely, we showed the following exciting results in our manuscript:
1. We obtained state-of-the-art performance on 102,855 images across 9 imaging modalities, significantly outperforming MedSAM (370 citations since 2024) and SAM (developed by META, 3,133 citations since 2023).  (Figure 2)
2. We showed that our method needs 430 times less user operations compared to MedSAM and SAM in cell segmentation. (Figure 2c)
3. Our tool is the first method that can detect irregular-shaped objects. (Figure 3)
4. Our tool can detect and reject invalid user requests, such as segmenting brain tissue in a chest X-ray. (Figure 2f-i)
5. Our tool is the first method that enables unsupervised object recognition, which simultaneously identifies and locates all objects in an image without any user-provided input. (Figure 4)
6. A case study showing the strong agreement between our method and pathologist annotation on three real-world patients collected from the Providence health care system. (Figure 5)

Based on these results, our manuscript has the following immediate implications:
1. Users can use our tool to analyze a large number of images, such as finding neoplastic cells in pathology images, with minimum effort.
2. Users can use our tool to detect complicated objects, such as vessels.
3. Users who do not have any domain expertise can use our tool without examining the image.
4. The model, code, and data will all be made publicly available, allowing continuing training of our model for specific user needs.

In summary, our method will revolutionize biomedical image analysis by allowing users to talk to the model in a hands-free manner. Please try our demo website at https://aka.ms/biomedparse-demo to further see how our GPT-4-based tool transforms biomedical image analysis.

Thank you for your consideration,
Hoifung Poon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\eat{
Background: Biomedical image analysis is fundamental for biomedical discovery. However, existing pipelines for biomedical image analysis are tedious and messy, since they often consist of multiple specialized tools, each responsible for a specific subtask. 

Key contribution: To address this long-standing problem, we developed BiomedParse, a biomedical imaging foundation model that simultaneously addresses image segmentation, object detection, and object recognition. BiomedParse is designed as a GPT-style chatbot that allows biologists to talk to the image for their needs. This is unprecedented because biologists no longer need to run any specialized software or label anything in the image (e.g., drag a bounding box). In fact, biologists can identify and locate all objects in the image without even taking a look at the image. Our model, for the first time, makes biomedical image analysis completely automated and intelligent. 

Key novelty: BiomedParse achieves this through a new foundation model paradigm called image parsing. In contrast to existing foundation model frameworks that are unsupervised, our image parsing framework explicitly considers supervised labels in the pre-training stage. This not only makes it more accurate but also enables it to analyze a new image with minimal or even zero user efforts, dramatically decreasing the user effort for all tasks in image analysis. 

Key technical advances: Image parsing used to be developed based on the Bayesian framework for image analysis 20 years ago, but was then quickly replaced by deep learning. We renovated image parsing by integrating GPT-4 into it, resulting in a model that can simultaneously understand images and text, corresponding to the "everything everywhere all at once" in our title.

Concretely, we showed the following exciting results in our manuscript:
1. We obtained state-of-the-art performance on 102,855 images across 9 imaging modalities, significantly outperforming MedSAM (370 citations since 2024) and SAM (developed by META, 3,133 citations since 2023).  (Figure 2)
2. We showed that our method needs 430 times less user operations compared to MedSAM and SAM in cell segmentation. (Figure 2c)
3. Our tool is the first method that can detect irregular-shaped objects. (Figure 3)
4. Our tool can detect and reject invalid user requests, such as segmenting brain tissue in a chest X-ray. (Figure 2f-i)
5. Our tool is the first method that enables unsupervised object recognition, which simultaneously identifies and locates all objects in an image without any user-provided input. (Figure 4)
6. A case study showing the strong agreement between our method and pathologist annotation on three real-world patients collected from the Providence health care system. (Figure 5)

Based on these results, our manuscript has the following immediate implications:
1. Users can use our tool to analyze a large number of images, such as finding neoplastic cells in pathology images, with minimum effort.
2. Users can use our tool to detect complicated objects, such as vessels.
3. Users who do not have any domain expertise can use our tool without examining the image.
4. The model, code, and data are all made publicly available, allowing continuing training of our model for specific user needs.

In summary, our method will revolutionize biomedical image analysis by allowing users to talk to the model in a hands-free manner. Please try our demo website at https://aka.ms/biomedseem-demo to further see how our GPT-4-based tool transforms biomedical image analysis.

Thank you for your consideration,
Hoifung Poon
}



==> nbt_sec/data_code.tex <==
\section*{Data availability}
\ourdata can be accessed at \oururl. The three real-world pathology images, including the annotations by pathologists and \ourmethod, can be accessed at \oururl. 

\section*{Code availability}
Our model can be accessed at \oururl, including the model weights and relevant source code. We include detailed methods and implementation steps in the Methods to allow for independent replication.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> results_arxiv.tex <==
\section*{Results}
\subsection*{Overview of \ourmethod and \ourdata}
To develop a model that can jointly solve segmentation, detection, and recognition, we need a supervision dataset that can cover all three tasks. To our knowledge, no existing large-scale biomedical image segmentation dataset contains the textual description for the structure of interests. To this end, we created the first such dataset \ourdata by integrating 45 biomedical image segmentation datasets and using GPT-4 to generate the textual description for each segmented object in each image. In particular, we utilized the data description and object type name (e.g., lower-grade glioma) to prompt GPT-4 for description generation (see \textbf{Methods}, \textbf{Supplementary Figure} \ref{fig:prompt}). To unify object types from these diverse datasets, we exploited GPT-4 to construct a three-layer ontology of segmentation objects (see \textbf{Methods}), spanning 3 main categories (histology, organ, abnormality), 15 meta-object types, and 82 specific object types (\textbf{Fig. \ref{fig1:overview}a}). In summary, \ourdata contains 6.77 million image-text pairs, spanning 9 imaging modalities and 25 anatomic sites (\textbf{Fig. \ref{fig1:overview}b, \textbf{Supplementary Figure} \ref{fig:data-modality-chord}}), representing a large-scale and diverse dataset for text-based biomedical image analysis. Although our method does not use bounding boxes, each image in \ourdata is associated with a bounding box, allowing us to evaluate traditional bounding-box-based approaches on it.

Building upon this dataset, we developed \ourmethod, a biomedical imaging foundation model that can jointly address segmentation, detection, and recognition in an image. In addition to being an all-in-one tool, \ourmethod needs much less user inputs compared to existing tools. The key idea of \ourmethod is to couple the shape and the textual description of an object type, allowing it to identify objects in an image by only using a textual description. This shift introduces unique challenges. First, the textual description, reflecting user intent, is not necessarily tailored to the given image. Second, a textual description could exhibit ambiguity due to linguistic variations. To address these issues, we exploit GPT-4 to generate variations of the input textual description in \ourdata according to the imaging modality and anatomic site (see \textbf{Methods}, \textbf{Supplementary Figures} \ref{fig:prompt} and \ref{fig:example}). 

Before evaluating image segmentation, we sought to examine the quality of embeddings derived from \ourmethod. We first compared the text embeddings from \ourmethod with the text embeddings from BiomedBERT \cite{gu2021domain}, the state-of-the-art language encoder in the biomedical domain. We found that embeddings from \ourmethod can better reflect cell types with a Silhouette score of 0.89, which is much higher than using the embeddings from BiomedBERT (\textbf{Fig. \ref{fig1:overview}d}, \textbf{Supplementary Figure} \ref{fig:ablation}). Next, we compared the image embeddings from \ourmethod with the image embeddings from Focal \cite{yang2022focal}, the state-of-the-art image encoder used to initialize our image encoder. We observed that embeddings from \ourmethod are more predictive of tumor cancerous on a pathology dataset \cite{glas} (\textbf{Fig. \ref{fig1:overview}e}). The superior performance of the text and image embeddings from our method necessitates the training of \ourmethod using \ourdata, raising our confidence that \ourmethod can be an effective approach for biomedical image analysis.



\subsection*{Accurate and scalable segmentation across 9 modalities}
We first evaluated \ourmethod on biomedical image segmentation on 102,855 holdout image-text pairs across 9 imaging modalities (\textbf{Fig. \ref{fig2:quant_eval}a}, \textbf{Supplementary Figure} \ref{fig:ablation}). We observed that \ourmethod achieved the overall best Dice score compared to the best-competing method MedSAM (paired t-test \textit{p}-value $< 10^{-4}$), demonstrating the effectiveness of our text-based framework. By comparing among existing approaches, we found that bounding box-based methods attained much higher performance than other text-based methods (e.g., Grounding DINO-based), demonstrating the difficulty of leveraging textual description for segmentation. Nevertheless, our method still outperformed existing bounding box-based methods, especially on modalities containing more irregular-shaped objects, such as pathology and CT. We also noticed that domain-specific methods, such as MedSAM, are better than general domain methods, necessitating the creation of our biomedical-specific dataset \ourdata for training domain-specific approaches. We highlighted a few examples showing the agreement between \ourmethod-derived segmentation and the ground truth segmentation across different modalities, demonstrating the generalizability of \ourmethod across modalities (\textbf{Fig. \ref{fig2:quant_eval}b}). We further compared \ourmethod on a benchmark created by MedSAM \cite{ma2024segment} encompassing 50 tasks and again observed the best performance by our method (paired t-test \textit{p}-value $< 10^{-2}$ ), reassuring the prominence of using text for image segmentation  (\textbf{Supplementary Figure} \ref{fig:overlap_eval_mod}).

In addition to being more accurate, our text-based segmentation approach is more scalable compared to bounding box-based approaches. This scalability is primarily due to the generalizability of textual descriptions across images of the same modality or anatomical site, eliminating the need for image-specific inputs. In contrast, bounding box-based approaches necessitate manual annotations for each image and each object, substantially increasing the workload of end users. To demonstrate this, we compared \ourmethod and the leading bounding box-based methods MedSAM and SAM on 42 colon pathology images for cell segmentation (\textbf{Fig. \ref{fig2:quant_eval}c}). By leveraging only one textual description ``glandular structure in colon pathology image'' for the entire dataset, \ourmethod achieves a 0.942 median Dice score, while neither SAM nor MedSAM achieves a median Dice score higher than 0.75. Furthermore, even when one ground truth bounding box for each image was provided, requiring 42 times more user operations, the median Dice scores of SAM and MedSAM didn't surpass 0.85. Notably, only when one bounding box was provided per cell (430 times more user operations), did MedSAM achieve a 0.969 Dice score that is slightly better than \ourmethod (\textbf{Fig. \ref{fig2:quant_eval}c}). Moreover, our results reveal that the bounding box-based approach is much less accurate on irregular-shaped objects, such as enhancing tumor and abnormal cells, in the one box per image setting (\textbf{Fig. \ref{fig2:quant_eval}d,e}). In contrast, our method still correctly segments these abnormal cells, suggesting better robustness against rare objects. The scalability of \ourmethod confirms its real-world utility by only requiring one user operation for an entire dataset.

Moreover, our method is capable of detecting invalid textual inputs, such as asking \ourmethod to segment a brain tissue in a chest X-Ray image, by calculating a \textit{p}-value using Kolmogorov–Smirnov (K-S) test (see \textbf{Methods}). We found that the invalid text has an average K-S test $p$-value smaller than $10^{-3}$ while the valid text has an average K-S test $p$-value of 0.123 (\textbf{Fig. \ref{fig2:quant_eval}f}). By using 0.01 as the p-value cutoff, \ourmethod can achieve a prominent detection performance of 0.93 precision and 1.00 recall on detecting invalid input (\textbf{Fig. \ref{fig2:quant_eval}g}). Moreover, we compared our method to Grounding DINO in invalid input detection and observed that Grounding DINO only achieves a median AUROC of 0.61 while \ourmethod attains 0.99, demonstrating our effectiveness in detecting invalid user text, serving as the basis for recognizing all objects in the image (\textbf{Fig. \ref{fig2:quant_eval}h,i}).


\subsection*{Accurate detection of irregular-shaped objects}
Next, we evaluated the performance of \ourmethod on object detection, where the model is asked to identify a queried object in the image. One advantage of \ourmethod is that it can take free text user queries that do not exactly match any object class. Since regular-shaped objects can be easily detected by our bounding box-free segmentation method, we focus on the more challenging case of detecting irregular-shaped objects and still use the Dice score as the evaluation metric. We hypothesize that our method can accurately detect irregular-shaped objects by mapping the semantic description to the object shape. To verify this, we illustrated the attribution map of each object learned by \ourmethod on the test data and observed that these attribution maps faithfully reflect object shapes, including many irregular-shaped objects (\textbf{Fig. \ref{fig3:irreg_eval}a}). Next, we define three metrics to assess the irregularity of an object, including \textit{convex ratio} (i.e., the ratio of the object size to the tightest convex size), \textit{box ratio} (i.e., the ratio of the object size to the tightest rectangle size), and \textit{rotational inertia} (i.e., the difficulty in changing the rotational velocity) (see \textbf{Methods}). We found that the improvements of \ourmethod over SAM and MedSAM are strongly correlated with these metrics (average correlation 0.829), indicating that our method has a larger improvement on irregular-shaped objects (\textbf{Fig. \ref{fig3:irreg_eval}b-d, Supplementary Figure \ref{fig:irregular_medsam}}). \textbf{Fig. \ref{fig3:irreg_eval}e} illustrates a few examples comparing our method and MedSAM on detecting irregular-shaped objects. Furthermore, \ourdata exhibits more irregularity than the datasets used by MedSAM (\textbf{Fig. \ref{fig3:irreg_eval}f,g}, \textbf{Supplementary Figure} \ref{fig:IRI_violin}), while the improvement of \ourmethod is also larger on \ourdata  (\textbf{Fig. \ref{fig3:irreg_eval}h}), reassuring the prominence of our method on detecting irregular-shaped objects. 

\subsection*{Object recognition using the segmentation ontology}
In our final analysis, we explore \ourmethod's capacity for object recognition, which aims to simultaneously segment and label every object within an image by only taking the imaging modality (eg., CT scans) as the input. To achieve this, \ourmethod utilizes our segmentation ontology to iteratively segment each pixel while enforcing spatial cohesion among adjacent pixels (see \textbf{Methods}). This approach enables \ourmethod to accurately conduct object recognition, as evidenced in \textbf{Fig. \ref{fig4:pano_eval}a}, where all objects are correctly identified and segmented with an average Dice score of 0.94. To systematically evaluate the performance of object recognition, we first calculated the precision and recall in terms of the objects that \ourmethod can correctly identify. We found that \ourmethod substantially outperformed the comparison approach Grounding DINO with a 25.0\%, 87.9\%, 74.5\% improvement on precision, recall, and F-1, respectively (\textbf{Fig. \ref{fig4:pano_eval}b-d}).  The improvement over comparison approaches is larger when more objects are present in the image (\textbf{Fig. \ref{fig4:pano_eval}e}). Next, we evaluated the performance of object recognition in terms of weighted average Dice score and found that our method again outperformed comparison approaches with a large margin (\textbf{Fig. \ref{fig4:pano_eval}f, Supplementary Figure \ref{fig:panoptic_scatter}}). Similar to our observation on object identification, the improvement over comparison approaches is larger when more objects are present in the image (\textbf{Fig. \ref{fig4:pano_eval}g}). These results indicate \ourmethod's ability to identify all objects in an image without any user input, offering a user-operation-free tool for biomedical image recognition.

Finally, we evaluated \ourmethod on real-world data of three patients collected from the Providence health care system (\textbf{Fig. \ref{fig5:prov_ex}}). We performed object recognition here by asking \ourmethod to label and segment all cell types without providing any inputs to it. We found that the annotations by \ourmethod are consistent with the pathologist annotations by correctly identifying regions of immune cells and cancer cells. While pathologists tend to focus on a specific region of cell type, our model can label all cells that match object types in our segmentation ontology, providing an efficient and effective tool for real-world clinical applications.   


